EdgeMatrix: A Resource-Redefined Scheduling Framework for SLA-Guaranteed Multi-Tier Edge-Cloud Computing Systems

With the development of networking technology, the computing system has evolved towards the multi-tier paradigm gradually. However, challenges, such as multi-resource heterogeneity of devices, resource competition of services, and networked system dynamics, make it difficult to guarantee service-level agreement (SLA) for the applications. In this paper, we propose a multi-tier edge-cloud computing framework, EdgeMatrix, to maximize the throughput of the system while guaranteeing different SLA priorities. First, in order to reduce the impact of physical resource heterogeneity, EdgeMatrix introduces the Networked Multi-agent Actor-Critic (NMAC) algorithm to re-define physical resources with the same quality of service as logically isolated resource units and combinations, i.e., cells and channels. In addition, a multi-task mechanism is designed in EdgeMatrix to solve the problem of Joint Service Orchestration and Request Dispatch (JSORD) for matching the requests and services, which can significantly reduce the optimization runtime. For integrating above two algorithms, EdgeMatrix is designed with two time-scales, i.e., coordinating services and resources at the larger time-scale, and dispatching requests at the smaller time-scale. Realistic trace-based experiments proves that the overall throughput of EdgeMatrix is 36.7% better than that of the closest baseline, while the SLA priorities are guaranteed still.

==> OverallAlgorithm.tex <==
\begin{algorithm}[t]
	\caption{The Overall Algorithm of \textit{EdgeMatrix}}
	\label{alg:OverallAlgorithm}
	Initialize the system environment\;
	Initialize training parameters\;
	Get the system observation $\hat{s}_{0}$\;
	\For{frame $\tau=0,1,2,...,$}
	{
		Get the actions of each agent $\hat{a}_{\tau}=\left(\hat{a}_{1,\tau},...,\hat{a}_{i,\tau},...\right)$\;
		Resource Customizer execution actions to get the redefined resources, cells and channels\;
		\For{channel $p=0,1,2,...,$}
		{
			Solve \textbf{JSORD} based on Algorithm\ref{alg:JSORD} in parallel on each channel $p\in\mathcal{P}$ \;
		}
		Get reward $\hat{r}_{\tau}$ and next observation $\hat{s}_{\tau+1}$\;
		Store sample data [$\hat{s}_{\tau},\hat{a}_{\tau},\hat{r}_{\tau},\hat{s}_{\tau+1}$] for updating neural network\;
		\If{frame \% update rate $==0$}
		{
			Update the parameters of actor ($\theta^{\mu}$) and critic($\theta^{\pi}$) using Eq. (\ref{equation:Critic update function}) and Eq. (\ref{equation:Actor update function})\;
			Save models.
		}
	}
\end{algorithm}



==> ServiceOrchestrationAlgorithm.tex <==
\begin{algorithm}[t]
	\caption{Solve JSORD Based on Submodular Function Maximization}
	\label{alg:JSORD}
	\KwIn{Input parameters of Eq. (1)\;} %
	\KwOut{Service orchestration variable $x^{\tau}_{p,l}$ and requests dispatch variable $y_{p,l,i,m}^{\tau}$\;}
	
	Initialize  $frame =\tau,\ channel=p$, $\mathcal{S} = \emptyset $, $T = \{e | e \in (\mathcal{L}_p\times \mathcal{M}_p) \setminus \mathcal{S}$, $\mathcal{S}\cup\{e\}$ satisfies constraints of (\ref{equation:7})$\}$ \;
    \While{$ T \neq \emptyset $}  
    	{  
    		$e^* = $ the element $e$ in $T$ that get the maximum value of \textit{\textbf{$\Omega(\mathcal{S}\cup\{e\}$}}\;
    		$\mathcal{S} = \mathcal{S}\cup \{e^*\}$\;
    		$T = \{e | e \in (\mathcal{L}_p\times \mathcal{M}_p) \setminus \mathcal{S}$, $\mathcal{S}\cup\{e\}$ satisfies constraints of (\ref{equation:7})\}\;
    	}
	Convert $\mathcal{S}$ to its vector representation $x^{\tau}_{p,l}$\;
	Compute $y_{p,l,i,m}^{\tau} = \{..., y_{p,l,i,m}^{t}, ...\}$ using Eq. (\ref{equation:6}) based on orchestrated services $x^{\tau}_{p,l}$\;
	\For{slot $t=0,1,2,...,$}
	{
		Execution request dispatch with dispatching variable $y_{p,l,i,m}^{t}$ at the small time scale.
	}


\end{algorithm}


==> TrainingAlgorithm.tex <==
\vspace{-0.3em}
\begin{algorithm}
	\caption{\small Training and Scheduling Process of \textit{KaiS}}
	\label{algorithm:global}
	\small Initialize the system environment and neural networks.
	
	
	\For{\rm{slot} $t$ = $1, 2, ...$}{

		
		\If {\rm{frame} $\tau$ \rm{begins}}{
			
			Get reward $\tilde{u}_{\tau-1}$ and store $[\tilde{\boldsymbol{s}}_{\tau-1}, \tilde{\boldsymbol{a}}_{\tau-1}, \tilde{u}_{\tau-1}] $;
			
			Use GNNs to embed system states as Eq. (\ref{equ:gnn embedding});
			
			Select $H$ high-value edge nodes $(\tilde{a}_{\tau}^{\bullet})$ and
			\linebreak compute their service scaling actions $(\tilde{\boldsymbol{a}}_{\tau}^{\star})$  \hspace*{3.0em}%
			\hbox{\raise 5pt \rlap{\smash{$\left.\begin{array}{@{  }c@{}}\\{}\\{}\\{}\\{}\\{}\\{}\\{}\end{array}\color{orchestrator2}\right\}$}}}
			\hbox{\raise 9pt \rlap{\smash{$\color{orchestrator2}\begin{tabular}{l}\rotatebox{270}{\footnotesize \textbf{\textit{Orchestrate (GPG)}}}\end{tabular}$}}} 
			\linebreak using policy networks $\theta_g$ and $\theta_q$, respectively;
			
			
			Execute orchestration action $\tilde{\boldsymbol{a}}_{\tau} = (\tilde{a}_{\tau}^{\bullet}, \tilde{\boldsymbol{a}}_{\tau}^{\star})$;
			
			Update GNNs and policy networks using Eq. (\ref{equ:GNNDRL policy gradient});
		}
		
		 \ForPar{\rm{each eAP agent} $b \in B$ }{
			
			\If{ $\mathcal{Q}_{b} == \varnothing$}{
			
				\textbf{Continue}
			}
			
			Update request queue $\mathcal{Q}_{b}$ and get reward $\hat{u}_{b, t-1}$;
			
			Store $[ \hat{\boldsymbol{s}}_{b, t-1}, \hat{a}_{b, t-1}, A\left(\hat{\boldsymbol{s}}_{b, t-1}, \hat{a}_{b, t-1}\right),\hat{u}_{b, t-1},$
			\linebreak $ \boldsymbol{F}_{b, t-1}] $ for $\theta_{p}$ (actor);
			
			Dequeue current request $r_{b, t}$; 
			
			Compute the resource context $\boldsymbol{F}_{b, t}$ using Eq. (\ref{equ:resource context});\hspace*{1.0em}%
			\hbox{\raise -5pt \rlap{\smash{$\left.\begin{array}{@{}c@{}}\\{}\\{}\\{}\\{}\\{}\\{}\\{}\\{}\\{}\end{array}\color{dispatchers2}\right\}$}}}
			\hbox{\raise -1pt \rlap{\smash{$\color{dispatchers2}\begin{tabular}{l}\rotatebox{270}{\textbf{\footnotesize \textit{Dispatch (cMMAC)}}}\end{tabular}$}}}
			
			Take dispatch action $\hat{a}_{b, t}$ for $r_{b,t}$ using Eq. (\ref{equ:probability of valid actions for agent});
			
		}
		
		Store $[ \hat{\boldsymbol{s}}_{t-1}, V^{*}\left(\hat{\boldsymbol{s}}_{t-1} ; \theta_{v}^{\prime}, \pi\right)] $ for $\theta_{v}$ (critic);
		
		Update neural networks $\theta_{p}$ (actor) and $\theta_{v}$ (critic) 
		\linebreak centrally using Eq. (\ref{equ:the gradient of policy of cMAAC}) and  (\ref{equ:loss function derived from Bellman equation}), respectively; 
		
		Synchronize $\theta_{p}$ periodically to distributed eAPs.
		
		
		
		
	} 
\end{algorithm}
\vspace{-0.6em}

